Improvements to Target-Based 3D LiDAR to Camera Calibration

The homogeneous transformation between a LiDAR and monocular camera is required for sensor fusion tasks, such as SLAM. While determining such a transformation is not considered glamorous in any sense of the word, it is nonetheless crucial for many modern autonomous systems. Indeed, an error of a few degrees in rotation or a few percent in translation can lead to 20 cm translation errors at a distance of 5 m when overlaying a LiDAR image on a camera image. The biggest impediments to determining the transformation accurately are the relative sparsity of LiDAR point clouds and systematic errors in their distance measurements. This paper proposes (1) the use of targets of known dimension and geometry to ameliorate target pose estimation in face of the quantization and systematic errors inherent in a LiDAR image of a target, and (2) a fitting method for the LiDAR to monocular camera transformation that fundamentally assumes the camera image data is the most accurate information in one's possession.

==> ProblemStatementANDLiDARTagPose.tex <==
\section{Problem Statement and Target Pose}
\label{sec:lidar}
This section describes what elements we need to solve the \lc~calibration problem,
\lidar's point clouds analysis, how to find 3D-2D correspondences and some important
things to keep in mind when doing \lc~calibration as specially \lidar's
irregular returns.


\subsection{Problem Statement}
The core of the problem is to
find a rigid body transform $H_L^C$ between a \lidar~and a camera, which
consists of 6 parameters, including a rotation
60
 matrix $\pre[L]R_L^C$ in $\SO(3)$ and
a translation $\pre[L]T_L^C$ in $\realnumbers^3$, where $\pre[L]R_L^C$ and
$\pre[L]T_L^C$ stands for the rotation and translation from a \lidar~ to a camera
represented in \lidar~frame, respectively. In target-based calibration, we need some
correspondences, features to match between a \lidar~and a camera. There are several
ways to represent features such as plane-line, plane-point, 3D line-line
correspondence or formulate as a Perspective-n-Point (PnP) problem. 

In this paper, we use fiducial tags to find correspondences in both 3D \lidar~point
cloud and in 2D images. Fiducial tags that detected from a \lidar~is called
\lidarts~and the same fiducial tags that detected from a camera is called \atags. A
pose of a \lidart~is provided from \red{cite}; the original method to obtain a
\lidart's pose, a transformation from \lidar~from to \lidart~frame $(H_L^T)$, is
running at realtime at 30 Hz; however, it is not accurate enough for calibration due
to noise level of \lidar~point cloud and thus has to be re-optimized mentioned in
Sec.~\ref{sec:lidartag_opt}. The noise level of \lidar~point cloud is discussed in
Sec.~\ref{sec:lidar_analysis}. Once the pose of the \lidart~is accurately obtained,
we then have 4 corners of the \lidart~in 3D. The same target in an image,  the 4
corners of the \atag~can be detected from \atag~detector in 2D. Therefore, this
allows us to have a set of 3D-2D correspondences on a target. The problem then
becomes a PnP optimization problem to compute a projection matrix mentioned in
Sec.~\ref{sec:extrinsic_opt}. However, this is not the end of the calibration. The
calibration up to this point assumes the corners given from \lidarts~are absolutely
correct. However the noise level of \lidar~point cloud, we still cannot fully trust
the optimization result of the \lidart. We have to do another refinement to the
\lidarts' poses given the projection matrix along with a regularizer mentioned in
Sec.~\ref{sec:refinement}.


\begin{remark}{
    \normalfont
One may argue why not directly using the optimized poses to do calibration, since two
poses from the two different sensors have been given already. It could be done easily
by: 
\begin{equation}H_L^C = H_L^{T_L} H_{T_L}^{T_C}\inv{\left(H_C^{T_{C}}\right)},
\end{equation} 
where $H_{T_L}^{T_C}$ is a
transformation from the \lidart~frame $(T_L)$ to the \atag~frame $(T_C)$. However,
this yet gives us good enough calibration result due to estimating an \atag~pose from
a monocular camera.}
\end{remark}

% In this paper, matrices and vectors are marked in bold. 
% $\prescript{}{L}{P}_A$ stands for a point A represented in \lidar frame. 
% A homogeneous transformation $\H$ consists of a rotation matrix $\pre[L]\R[L][T]$ and a translation vector
% $\pre[L]\T[L][T]$: $$\H[L][T] = \begin{bmatrix}\pre[L]\R[L][T] & \pre[L]\T[L][T] \\
% \zeros &1\end{bmatrix},$$

\subsection{\lidar~Point Cloud Analysis}
\label{sec:lidar_analysis} 
\lidars~have dense region and sparse region on the z-axis as shown in Fig.~\red{dense
region}. We use a 32-beam Velodyne Ultra Puck, the resolution on z-axis is
\red{number} and \red{number} of the dense region and the sparse region respectively.
The points resolution on the y-axis is \red{number}. The quantization error on both
y-axis and z-axis direction could be roughly computed from: As a result, the
quantization error could get quite large if one place the tag at a far distance.
In Fig.~\red{Calibration error} shows if we have 1 degree on each axis and 5\% of
translation error, the calibration result is not good enough for our application.
Thus, it is essential to use geometry constraint to estimate a \lidart~pose as well as
to place a \lidart~at a tilted angle so that the geometry constraint can pick up the
quantization error on y-axis and z-axis. To overcome quantization error on x-axis, we
accumulate a few scans to estimate one \lidrt~pose and condition on the current
estimate of projection matrix to refine the \lidart's poses mentioned in
Sec.~\ref{sec:refinement}.



\subsection{Correspondences and Automatic Detection}
\label{sec:correspondences}
\subsubsection{\lidart~Poses Optimization and Automatic Detection}
\label{sec:lidartag_opt}
To find 3D correspondences in \lidar~point cloud, we use corners of a \lidart~as our
\lidar~target. Patches \lidarts' point clouds are automatically detected from a full
scan of point cloud by \red{cite} and therefore we can assume they are given in this
paper. When estimating a \lidart' pose using its centroid and a normal vector
computed by taking svd of the \lidart's points (more detail, please refer to
\red{cite}), which is fast and suitable for realtime application; however, we notice
there are observable noise of the normal vector and centroid. We further look into
the \lidart~points; we observe the points on the \lidart, a planner object, they
appears as a cube, as shown in Fig.~\red{lidartag cube}. The min/max of the
difference of depth could be 5 cm to 15 cm on x-axis direction; the standard
deviation is also noticeable as shown in Table.~\red{payload point analysis}. The
orientation also has a few degree of variance. As shown in Fig.~\red{calibration
error}, this error is large enough to ruin the calibration. To more accurately
estimate a \lidart~pose, we formulate another optimization problem that does not use
its centroid nor normal vector but take into account its underline noise.

We place an ideal reference target at the center of the \lidar~frame as shown in
Fig.~\red{reference frame}. We want to find the best homogeneous transformation
$H_T^L$ that takes the \lidart~''back'' to the ideal reference target. To do so, we
define a cost function based upon the known geometry (diamond), size (d) and the
noisy level on x-axis (k) of the \lidart. Given a set of \lidart's point cloud
$\pre[L]X_i(x_i, y_i, z_i)$ , 8 corners of the ideal reference frame $\pre[L]Y_i^\prime$,
and the current estimate of $\pre[L]\tilde{R}_T^L$ and $\pre[L]\tilde{T}_T^L$ the
cost for the \lidart's point cloud is defined as: 

% \begin{align}
%     c(X) = \sum_{i=1}^{N} 
%     &\min\left(||x_i- \frac{0.01}{2}||^p, ||x_i-\frac{0.01}{2}||^p\right) + \\
%     &\min\left(||y_i- \frac{d}{2}||^p, ||(y_i- \frac{-d}{2}||^p\right) + \\
%     &\min\left(||z_i- \frac{d}{2}||^p, ||(z_i- \frac{-d}{2}||^p\right).
% \end{align}
% \begin{align}
%     c(X, \widetilde{R_T^L}, \widetilde{T_T^L}) = \sum_{i=1}^{N} &c_x(x_i, \widetilde{R_T^L}_{1,:}, \widetilde{T_L^T}_{1}) + \\
%                                                                 &c_y(y_i, \widetilde{R_T^L}_{2,:}, \widetilde{T_L^T}_2) + \\
%                                                                 &c_z(z_i, \widetilde{R_T^L}_{3,:}, \widetilde{T_L^T}_3),
% \end{align}
\begin{equation}
    \pre[L]\tilde{X_i} = \left(\pre[L]\tilde{R}_T^L\right)\left(\pre[L]X_i\right) + 
    \pre[L]\tilde{T}_T^L
\end{equation}
\begin{equation}
    C(\pre[L]\tilde{X}) = \sum_{i=1}^{N} &c_x(\tilde{x}_i) + \\
                                  &c_y(\tilde{y}_i) + \\
                                  &c_z(\tilde{z}_i),
\end{equation}
% where $\widetilde{R_T^L}, \widetilde{T_T^L}, c_x(x), c_y(y)$ and $c_z(z)$ are:
% \begin{equation}
%     \widetilde{R_T^L} = \begin{bmatrix} \widetilde{R_T^L}_1\\ \widetilde{R_T^L}_2 \\ \widetilde{R_T^L}_3\end{bmatrix}
% \end{equation}
where $c_x(\tilde{x}), c_y(\tilde{y})$ and $c_z(\tilde{z})$ are:
% \scalebox{0.9}{%
 \begin{equation}
% c_x(x_i, \widetilde{R_T^L}_{1,:}, \widetilde{T_L^T}_{1}) =
     c_x(\tilde{x}_i) =
    \begin{cases}
        \min\left(||\tilde{x}_i- \frac{k}{2}||^p, ||(\tilde{x}_i- \frac{-k}{2}||^p\right), & 
        \text{if } \frac{-k}{2}\leq \tilde{x}_i \leq \frac{k}{2}\\\
        0, & \text{otherwise}.
    \end{cases}
\end{equation}
%}
\begin{equation}
    c_y(\tilde{y}_i) = 
    \begin{cases}
        \min\left(||\tilde{y}_i- \frac{d}{2}||^p, ||(\tilde{y}_i- \frac{-d}{2}||^p\right), & 
        \text{if } \frac{-d}{2}\leq \tilde{y}_i \leq \frac{d}{2}\\\
        0, & \text{otherwise}.
    \end{cases}
\end{equation}
\begin{equation}
    c_z(\tilde{z}_i) = 
    \begin{cases}
        \min\left(||\tilde{z}_i- \frac{d}{2}||^p, ||(\tilde{z}_i- \frac{-d}{2}||^p\right), & 
        \text{if } \frac{-d}{2}\leq \tilde{z}_i \leq \frac{d}{2}\\\
        0, & \text{otherwise}.
    \end{cases}
\end{equation}
The optimal $H_T^L^*$ can be determined:
\begin{align}
    H_T^L^* &= \argmin_{\pre[L]\tilde{R}_T^L, \pre[L]\tilde{T}_T^L}
    C(\pre[L]\tilde{X}, \pre[L]\tilde{R}_T^L, \pre[L]\tilde{T}_T^L)\nonumber \\ &=
    \argmin_{\pre[L]\tilde{R}_T^L, \pre[L]\tilde{T}_T^L} \sum_{i=1}^{N} c_x(\tilde{x}_i) +
    c_y(\tilde{y}_i) + c_z(\tilde{z}_i).
\end{align}

Conceptually, if a transformed point is inside the ideal reference frame, the cost is zero;
otherwise, we penalize its each axis with p-norm to a closest boundary of the ideal reference
frame along the same axis. In this work, we choose L1-norm and we find this cost is also robust
to outliers as shown in Fig.\red{robust to outliers}.

We now have an optimized $H_T^L$, a transformation from a \lidart~frame to the ideal
reference frame and we also have the 8 corners of the ideal reference target
$\pre[L]Y_i^\prime$. We can compute the 8 corners \footnote{These 8 corners are two
planes with geometry constraints; we can take the average of the two planes to
find the neutral plane with 4 corners.} of the \lidart~($\pre[L]Y_i$) easily by:
\begin{equation}
    \pre[L]Y_i = \inv{\left(H_T^L\right)} \pre[L]Y_i^\prime,
\end{equation}
where these corners will be refined again after the projection matrix is estimated.

\subsubsection{Image correspondences from \atags}
\label{sec:apriltag_correspondences}
Getting corners correspondence from the same fiducial tag in an image is fairly
easier and straight forward. The corners of the fiducial tag in an image, namely an
\atag, can be automatically detected by the \atag detector. In original
papers\cite{olson2011apriltag}, \cite{wang2016apriltag}, \cite{krogiusflexible}, the corners are defined at the payload corners\footnote{The
detector finds four-sided regions that have darker interior than their exterior in
the whole image.}, shown in Fig.~\red{payload explain}. However, we can use the detected
corners and tag-relative coordinates to backstep to the outer 4 corners $\pre{C}Y_i$.


==> Related.tex <==
\section{Related Work}
\label{sec:related_work}
